Algorithmic Collusion Without Threats

There has been substantial recent concern that pricing algorithms might learn to ``collude.'' Supra-competitive prices can emerge as a Nash equilibrium of repeated pricing games, in which sellers play strategies which threaten to punish their competitors who refuse to support high prices, and these strategies can be automatically learned. In fact, a standard economic intuition is that supra-competitive prices emerge from either the use of threats, or a failure of one party to optimize their payoff. Is this intuition correct? Would preventing threats in algorithmic decision-making prevent supra-competitive prices when sellers are optimizing for their own revenue? No. We show that supra-competitive prices can emerge even when both players are using algorithms which do not encode threats, and which optimize for their own revenue. We study sequential pricing games in which a first mover deploys an algorithm and then a second mover optimizes within the resulting environment. We show that if the first mover deploys any algorithm with a no-regret guarantee, and then the second mover even approximately optimizes within this now static environment, monopoly-like prices arise. The result holds for any no-regret learning algorithm deployed by the first mover and for any pricing policy of the second mover that obtains them profit at least as high as a random pricing would -- and hence the result applies even when the second mover is optimizing only within a space of non-responsive pricing distributions which are incapable of encoding threats. In fact, there exists a set of strategies, neither of which explicitly encode threats that form a Nash equilibrium of the simultaneous pricing game in algorithm space, and lead to near monopoly prices. This suggests that the definition of ``algorithmic collusion'' may need to be expanded, to include strategies without explicitly encoded threats.

==> abstract.tex <==
There has been substantial recent concern that automated pricing algorithms might learn to ``collude.''  Supra-competitive prices can emerge as a Nash equilibrium of repeated pricing games, in which sellers play strategies which threaten to punish their competitors if they ever ``defect'' from a set of supra-competitive prices, and these strategies can be automatically learned. But threats are anti-competitive on their face. In fact, a standard economic intuition is that supra-competitive prices  emerge from \emph{either} the use of threats, \emph{or} a failure of one party to correctly optimize their payoff. Is this intuition correct? Would explicitly preventing threats in algorithmic decision-making prevent supra-competitive prices when sellers are optimizing for their own revenue?  

No. We show that supra-competitive prices can robustly emerge even when both players are using algorithms which do not explicitly encode threats, and which optimize for their own revenue. Since deploying an algorithm is a form of commitment, we study sequential Bertrand pricing games (and a continuous variant) in which a first mover deploys an algorithm and then a second mover optimizes within the resulting environment. We show that if the first mover deploys \emph{any} algorithm with a no-regret guarantee, and then the second mover even approximately optimizes within this now static environment, monopoly-like prices arise. The result holds for any no-regret learning algorithm deployed by the first mover and for \emph{any} pricing policy of the second mover that obtains them profit at least as high as a random pricing would --- and hence the result applies even when the second mover is optimizing only within a space of non-responsive pricing distributions which are incapable of encoding threats. In fact, there exists a set of strategies, neither of which explicitly encode threats that form a Nash equilibrium of the simultaneous pricing game in algorithm space, and lead to near monopoly prices. This suggests that the definition of ``algorithmic collusion'' may need to be expanded, to include strategies without explicitly encoded threats.

==> experiments.tex <==
\section{Numerical Investigation of Constants}
\label{sec:experiments}
%\esh{is responsible for this section}

%\esh{Things to add: Interpret the Stackelberg value explicitly}

%\jz{Can we make the figures smaller and in fact even side-by-side? Kind of "ugly" right now}
%\esh{They are? the figures are beautiful to my eyes:(.  Jokes aside, are they thematically similar enough? One is about establishing a pattern about the Stackelberg payoffs with changing $k$ while the other aims to give some idea about the the Stackelberg strategy for a fixed $k$.}
%\jz{\url{https://www.youtube.com/watch?v=oofSnsGkops}}
%\jz{yeah the common theme is the structure of the stackelberg and the left and right side highlight different aspects, with subcaptions}
We showed in Lemma~\ref{lemma:uniform_is_good_enough} that the optimizer can get a payoff of $\Omega_k(T)$ against any no-regret learner, just by playing the uniform distribution over their prices. An implication is that they would do at least as well with their optimal static strategy, which was enough for our results which are stated in asymptotic notation. While we did not get attractive constants via this simple approach, we numerically verified that the optimal static optimizer distribution against a no-regret algorithm, which is the Stackelberg leader strategy for a number of values of $k$, results in average prices of more than $\frac{2}{3}$ (in fact approximately $\frac{2(k-1)}{e k}$). ~\cite{conitzer2006computing} give an efficient algorithm for computing the Stackelberg equilibrium of a two player game, which we use to numerically compute the Stackelberg leader strategy as well as the payoff of the Stackelberg leader, which will approximately (up to subconstant in $T$ additive error) be the average payoff of the optimizer repeatedly playing the Stackelberg leader strategy (using Lemma~\ref{lemma:fixed_strategy_nr}). Our numerical results show that the Stackelberg value of the leader (as well as the follower) is approximately $\frac{k-1}{ek}$ for a range of values of $k$ in Figure~\ref{fig:payoff_growth}. By Observation~\ref{obs:value_transfer}, if the follower optimizes over the space of static strategies, the average price for the buyer will be $\frac{2(k-1)}{ek} \geq \frac{2}{3}$. We note that while our experiments show these prices are achievable by non-responsive optimizers for all values of $k$ from $1$ to $200$, it remains interesting future work to prove that this holds for all $k$. Finding a closed form analytical expression for the Stackelberg leader strategy of the stage game is an open problem and would likely help in proving the conjecture for all  $k$.



\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/newmodel_trajectory.png}
        \caption{Stackelberg Leader/Follower Payoffs for varying $k$}
        \label{fig:payoff_growth}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/stack_strategy_leader_100.png}
        \caption{Stackelberg Leader Strategy for $k=100$.}
        \label{fig:stack_100}
    \end{subfigure}
    %\caption{Comparison of Stackelberg Leader and Follower Payoffs and Leader Strategy for different values of $k$}
    \label{fig:combined_stackelberg}
\end{figure}

\begin{comment}
    

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/newmodel_trajectory.png}
    \caption{Stackelberg Leader and Follower Payoffs for varying price discretization $k$}
    \label{fig:payoff_growth}
\end{figure}

\end{comment}

We also show the Stackelberg strategy for $k=100$ in Figure~\ref{fig:stack_100}. Our numeric results also indicate that every price between $36/100$ to $98/100$ is (tied for being) a best response for the follower given the optimal leader commitment\footnote{In the Stackelberg Equilibrium problem, the follower typically tie-breaks in favor of the leader, in our application the optimizer adds some infinitesimal extra probability mass on price $ 99/100$ to ensure that no-regret learner learns a unique best-response of $98/100$ (which is the best outcome for the optimizer).}.

\section{Discussion and Conclusion}
Defining anti-competitive behavior is delicate. Monopoly like prices can arise in a number of scenarios: a \emph{failure to optimize} (if e.g. players are simply not best responding to one another) as well as through \emph{collusion} (which has been interpreted as requiring explicit \emph{threats} when speaking of algorithmic collusion \cite{calvano20,harrington}). Past work \cite{hartline2024regulation,chassang23} have proposed no-swap-regret algorithms as reasonable competitive algorithms in pricing scenarios, on the basis that they converge to competitive prices when both parties use them, and they seem both to successfully optimize and not to encode threats. 

Our results complicate this picture. We show that if the first entrant into a market deploys a pricing algorithm with the no-swap-regret guarantee, then this very strongly incentivizes the next entrant to deploy an algorithm that will lead to supra-competitive prices. In fact, \emph{anything the second entrant does} that obtains them profit at least that of a random pricing strategy will inevitably lead to supra-competitive prices. Moreover, this will not be at the expense of the first entrant---the no(-swap) regret learner will \emph{also} enjoy supra-competitive revenue. And the algorithm of the second entrant can be entirely static and non-responsive, and therefore unable to encode threats. In fact, this phenomenon does not hinge on the sequential nature of play that we focus on and does not hinge on either player having commitment power. As we show, there is a Nash equilibrium of the game---in algorithm space---maintaining supra-competitive prices, which involves one player playing a no swap regret algorithm and the other playing a static pricing distribution. Both players are best responding to one another in the space of all pricing algorithms (without any restriction) and so neither player is failing to optimize---but neither are either of the players deploying threats. We suggest that this might require a reconsideration of what constitutes algorithmic collusion.


\begin{comment}
    

%\esh{This figure can be unchanged, since the x axis is indices, not the prices themselves}
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/stack_strategy_leader_100.png}
    \caption{Stacklerberg Leader Strategy for $k=100$}
    \label{fig:stack_100}
\end{figure}
\end{comment}
%\subsection{Proof of Lemma~\ref{lemma:ce_competitive}}
%\label{sec:ce_competitive}

==> generalized_results.tex <==
\section{Generalized Model Results}



The plan is to prove a few operational lemmas about the nature of the stage game under the generalized model, and then rewrite the four main results in the Bertrand duopoly in terms of just these lemmas.

\begin{lemma}
\label{lemma:lower_br}
Fix the strategy of agent $2$ to picking price $p$ with $p \ge 3$ \esh{(or some constant depending on $\lambda$)}, then agent $1$'s best-response $BR(p)$ (with arbitrary tie-breaking) satisfies $BR(p) < p$ and $BR(p) = \Omega(p)$.
\end{lemma}


\begin{proof}
    {\bf Part 1:} $BR(p) < p$. 
    
    By responding with price $x$, agent 1's payoff is $x \cdot W(x,p)$.
    Let us consider a proxy winner function $W'$ defined below:

    \[ 
    W'(x,p) = \begin{cases}
    \min \left \{\frac{1}{2} + \lambda \left(1 - \frac{x}{p} \right), 1 \right \} \quad \text{where $x \le p$ , $p \in [k]$},\\
        \max \left \{ \frac{1}{2} - \lambda \left(1 - \frac{p}{x} \right), 0 \right \} \quad \text{ where $x \ge p$. }
    \end{cases}
    \]

    By construction, we have $W(x,p) \ge W'(x,p)$ where $x \le p$ and $W(x,p) \le W'(x,p)$ where $x \ge p$. Thus, showing $BR(p) < p$ under this winner function $W'$ will automatically imply the result for $W$.

    Define $\beta := \left( 1 - \frac{1}{2\lambda} \right )$. Since $\lambda > \frac{1}{2}$, $\beta$ is a constant with $\beta \in (0,1)$. Let $f(x) :=  x \cdot W'(x,p)$ denote agent 1's payoff by playing $x$ against $p$ under the winner function $W'$. 

    \[ 
    f(x) = \begin{cases}
        x, \quad x \le p \cdot \beta \\
        x \left \{\frac{1}{2} + \lambda \left(1 - \frac{x}{p} \right)\right \}, \quad x \in [p \cdot \beta, p] \\
        x  \left \{ \frac{1}{2} - \lambda \left(1 - \frac{p}{x} \right) \right \} \quad x \in [p, \frac{p}{\beta}]\\
        0, \quad x \ge \frac{p}{\beta}
    \end{cases}
    \]


    We can also generate the derivative of each piece of the function:

\[ 
    f'(x) = \begin{cases}
        1, \quad x < p \cdot \beta \\
        \frac{1}{2} + \lambda - \frac{2 \lambda x}{p}, \quad x \in (p \cdot \beta, p) \\
        \frac{1}{2} - \lambda, \quad x \in (p, \frac{p}{\beta})\\
        0, \quad x \ge \frac{p}{\beta}
    \end{cases}
    \]

    It is easy to see that the payoff function is maximized uniquely at $x = \left (\frac{1}{4 \lambda} + \frac{1}{2} \right) p $, which is strictly less than $p$ since $\lambda > \frac{1}{2}$.

    \esh{Some issues with discretization here, but I think we can skirt them by only working with large enough $p$  and increasing the lower bound on $\lambda$}

    {\bf Part 2:} $BR(p) = \Omega(p)$. We know that responding with price $x' = \floor { p \cdot \beta}$ is better than any other lower price since $W(x,p) = 1$ if $x \le x'$. This directly implies the desired result.
    
\end{proof}



\begin{lemma}
\label{lemma:dist_lower_br}
Fix any distribution $X$ of agent $2$ supported on prices up to and including $p$ with $p \ge 3$ \esh{(or some constant depending on $\lambda$)}, then agent $1$'s best-response $BR(X)$ (with arbitrary tie-breaking) satisfies $BR(p) < p$ ,$BR(p) = \Omega(p)$. In particular, $BR(p)$ obtains some constant improvement over any response that is greater than or equal to $p$.
\end{lemma}

\begin{proof}
    
\end{proof}


